Inferring Global Exponential Stability Properties using Lie-bracket Approximations

In the present paper, a novel result for inferring uniform global, not semi-global, exponential stability in the sense of Lyapunov with respect to input-affine systems from global uniform exponential stability properties with respect to their associated Lie-bracket systems is shown. The result is applied to adapt dither frequencies to find a sufficiently high gain in adaptive control of linear unknown systems, and a simple numerical example is simulated to support the theoretical findings.

==> src/sections/auxiliary-results/00--auxiliary-results.tex <==
This section contains the auxiliary statements needed for the functional expansion.


\input{assumptions/mixed.tex}

\input{src/lemmata/new-functional-expansion.tex}

% \input{include/lemmata/auxiliary-bounds-common.tex}
% \input{include/lemmata/auxiliary-bounds-QV1.tex}
% \input{include/lemmata/auxiliary-bounds-QV2.tex}
% \input{include/lemmata/auxiliary-bounds-Q1T.tex}
% \input{include/lemmata/auxiliary-bounds-Q1.tex}
% \input{include/lemmata/auxiliary-bounds-H.tex}
% \input{include/lemmata/auxiliary-bounds-I.tex}
% \input{include/lemmata/auxiliary-bounds-RL1.tex}
% \input{include/lemmata/auxiliary-bounds-RT1.tex}
% \input{include/lemmata/auxiliary-bounds-R.tex}
% \input{include/lemmata/auxiliary-bounds-J0.tex}
% \input{include/lemmata/auxiliary-bounds-Jij.tex}

% \input{include/lemmata/lipschitz-properties-1.tex}
% \input{include/lemmata/lipschitz-properties-2.tex}
% \input{include/lemmata/lipschitz-properties-3.tex}

==> src/sections/auxiliary-results/base-assumptions.tex <==
\begin{assumption}[Base Assumptions]\label{ass:base}
	Consider system~\eqref{eqn:es-system}. Suppose that \Cref{ass:fi,ass:ui} hold.
	Let \( t_0 \in \mathbb{R}\), \( t_1 \in \interval[open]{t_0}{\infty}\), \( \omega_1 \in \interval[open right]{1}{\infty}\), \( \Lambda_3 \in \interval[open right]{1}{\infty} \) and \( x_0 \in \mathbb{R}^n\), such that the trajectory \( x_{\omega_1}(t; t_0, x_0)\) of~\eqref{eqn:es-system} through \( x(t_0) = x_0\) exists on \( \interval[]{t_0}{t_1} \) and satisfies
	\begin{align}
		\| x_{\omega_1}(t; t_0, x_0) \| & \leq \Lambda_3 \|x_0\|
	\end{align}
	\hfill for all \( t \in \interval[]{t_0}{t_1}\).
\end{assumption}

==> src/sections/proofs/00--proofs.tex <==
The fully elaborated versions of the proofs are given in \cite{webergharesifardebenbauer2023}.

% \subsection{Proofs of Main Results}
% \pagebreak
% \printProofs[main-result]
% \vfill
\begin{proof}[of \Cref{lemma:approximation-lemma}]\label{proof:approximation-lemma}
  In virtue of \Cref{ass:ui,ass:fi}, the Picard-Lindel{ö}f Theorem guarantees the global existence of solutions \(x_\omega(t; t_0, x_0)\) to \eqref{eqn:es-system} for every \( t_0 \in \mathbb{R} \), \( x_0 \in \mathbb{R}^n \) and \( \omega \in \interval[open]{0}{\infty}\).
  
  % the following are satisfied:
  % \begin{enumerate}%[
  %   % wide,
  %   % itemindent=!,
  %   % labelindent =\parinddent,
  %   % labelwidth=0pt,
  %   % listparindent=\parindent,
  %   % align=left,
  %   % label={\scriptsize(\arabic*)},
  %   %  leftmargin=0pt
  %   % ]
  %   \item The pair \((\mathbb{R}^n, \norm{\cdot})\) forms a Banach space.
  %         % \item For every \( (t_0, x_0) \in \mathbb{R} \times \mathbb{R}^n \), the function \( f(t_0, x_0) : \mathbb{R} \times \mathbb{R} \to \mathbb{R} \) is measurable.
  %   \item The vector field			     \( f_{\omega}(t, x)  \coloneqq  \sum_{i=0}^l \omega^{p_i} f_i(t, x) \cdot u_i(\omega t) \)
  %         is continuous, and uniformly globally Lipschitz on \( \mathbb{R} \times \mathbb{R}^n\).
  % \end{enumerate}
  % Consequently, the Picard-Lindel{ö}f Theorem guarantees, that for every \( t_0 \in \mathbb{R} \), \( x_0 \in \mathbb{R}^n \) and \( \omega \in \interval[open]{0}{\infty}\), there exists a \( t_u(t_0, x_0, \omega) \in \interval[open]{0}{\infty}  \) such that the trajectory of system~\eqref{eqn:es-system} with initial condition \( x(t_0) = x_0 \) exists uniquely on \( \interval[]{t_0}{t_0 + t_u(t_0, x_0, \omega)} \).
  % Let \( t_m(t_0, x_0, \omega)\) be the supremal value of \( t_u(t_0, x_0, \omega)\).
  % Since \(f_\omega\) is uniformly \emph{globally} Lipschitz, the solution exists globally and \( {t_m = \infty}\).
  
  
  Observe, that both solutions \( x_{\omega}\) and \( \bar{x}\) exist {(at least)} on their common interval \(  \mathcal{T}(t_0, x_0, \omega) \coloneqq \interval[]{t_0}{t_0+t_f} \cap \interval[]{t_0}{t_0+ t_m(t_0, x_0, \omega)} = \interval[]{t_0}{t_0+t_f}\) per assumptions of this theorem.
  
  
  To prove the result, let us proceed by contradiction. Namely, let us falsify the following statement obtained by negating a portion of the statement of this theorem:
  
  \begin{customassumption}[Contradiction Statement]\label{ass:contradiction-assumption}
    Let \( D \in \interval[open]{0}{\infty}\) be arbitrary but fixed.
    % Suppose the assumptions of this lemma hold, and let \(\omega^\star\) as defined in~\eqref{eqn:def:omega-star}.
    Then for each \( \omega^\star \in \interval[open]{0}{\infty}\), there exists an \({ \omega_1 \in \interval[open]{\omega^\star}{\infty}}\),  \({ t'_0 \in \mathbb{R}} \), a~\( {x'_0 \in {\mathbb{R}^n \! \setminus \!\set{0}}} \) and  \({ t_s \in \mathcal{T}(t'_0, x'_0, \omega_1)}\), such that the trajectories of systems~\eqref{eqn:es-system} and~\eqref{eqn:lbs} through \({ x(t'_0) = x'_0 }\) and \( {\bar{x}(t'_0) = x'_0}\) satisfy
    % \begin{align*}
    % 	\norm{ x_{\omega_1}(t_s; t'_0, x'_0) - \bar{x}_{\omega_1}(t_s; t'_0, x'_0) } \geq D \norm{x_0'} .
    % 	\qedhere
    % \end{align*}
    \par
    \vspace{\abovedisplayskip}
    \hfill \(\displaystyle \norm{ x_{\omega_1}(t_s; t'_0, x'_0) - \bar{x}(t_s; t'_0, x'_0) } \geq D \,\norm{x_0'} \) \;. \qedhere
  \end{customassumption}
  
  Let \( D \) be arbitrary but fixed. For (\nameref{ass:contradiction-assumption}) to hold for all \( \omega^\star \in \interval[open]{0}{\infty}\), it must hold in particular for \( \omega^\star\) as defined in~\eqref{eqn:def:omega-star}.
  
  
  Note that \( x_{\omega_1}(t; t'_0, x'_0) \) and \( \bar{x}(t; t'_0, x'_0) \) are absolutely continuous on \( \interval[]{t'_0}{t_s} \).
  According to (\nameref{ass:contradiction-assumption}), having \( \norm{ x_{\omega_1}(t_s; t'_0, x'_0) - \bar{x}(t_s; t'_0, x'_0) } \geq D \norm{x_0'} \) with \({ \norm{ x_{\omega_1}(t'_0; t'_0, x'_0) - \bar{x}(t'_0; t'_0, x'_0) }  = 0} \) implies the existence of a \( t_2 \in \interval[open left]{t_0'}{t_s} \), such that
  \begin{subequations}
    \begin{align}
      \norm{ x_{\omega_1}(t_2; t'_0, x'_0) - \bar{x}(t_2; t'_0, x'_0) } & = D \, \norm{x_0'} %\qquad\text{and}
      \label{eqn:tmp:pfe:ca:1}
    \end{align}
    and
    \begin{align}
      \norm{ x_{\omega_1}(t; t'_0, x'_0) - \bar{x}(t; t'_0, x'_0) } & < D \, \norm{x_0'}      \label{eqn:tmp:pfe:ca:2}
    \end{align}
    for all \( t \in \interval[open right]{t'_0}{t_2} \).
  \end{subequations}
  To reach a contradiction, we will now examine the distance between \(x_{\omega_1}(t; t'_0, x'_0)\) and \(\bar{x}(t; t'_0, x'_0)\).
  Let \( t_1 \in \interval[]{t'_0}{t_2} \) be arbitrary but fixed.
  Since \( \bar{x}(t; t'_0, x'_0)\) exists on \( \interval[]{t'_0}{t_1}\), we may express the solution to~\eqref{eqn:lbs} as
  \begin{align}
    \begin{split}
      \MoveEqLeft
      \bar{x}(t_1; t'_0, x'_0)
      ={}  x'_0 + \int_{t'_0}^{t_1} f_0(\theta, \bar{x}(\theta; t'_0, x'_0))
      \\
       & + \sum_{\mathclap{\substack{1\leq i <l \\i<j \leq l}}} \;
      \lim_{\omega \to \infty}
      \commutator{f_i}{f_j}(\theta, \bar{x}(\theta; t'_0, x'_0)) \gamma_{ij}(\omega) \odif{\theta}.
    \end{split}
    \label{eqn:A68}
  \end{align}
  Furthermore, since the conditions of \Cref{lemma:functional-expansion} are met with the selected values of \(\omega_1\), \(t_0 = t'_0\), \(t_1\) and \(x_0 = x'_0\) and the choice of \(  D \), we may express the solution to~\eqref{eqn:es-system} according to \Cref{lemma:functional-expansion}
  % \begin{align}
  %   \begin{split}
  %     \MoveEqLeft
  %     x_{\omega_1}(t_1; t'_0, x'_0)
  %     =
  %     x'_0
  %     % \\
  %     % &
  %     + \int_{t'_0}^{t_1} f_0(\theta, x_{\omega_1}(\theta; t'_0, x'_0))
  %     \\
  %      & + \sum_{\mathclap{\begin{limitarray}
  %                                    1 &\leq i &< l \\
  %                                    i&<j&\leq l
  %                                  \end{limitarray}}} \commutator{f_i}{f_j}(\theta, x_{\omega_1}(\theta; t'_0, x'_0)) \gamma_{ij}(\omega) \odif{\theta} \\
  %      & + \sum_{q=0}^{r-1} \!R(t'_q, t'_{q+1}) + \!R(t'_b, t_1) + \!R_{T_1}(t'_0, t_1),
  %   \end{split}
  %   \label{eqn:A69}
  % \end{align}
  with \( T_1\), \( r  \), \( t_q\), \(R\) and \( R_{T_1}\) defined in \Cref{ass:functional-expansion}.
  Combining~\eqref{eqn:A68} with~\eqref{eqn:functional-expansion:main}, we obtain with
  \begin{subequations}
    \begin{align}
      J_0(\theta)     \coloneqq{} & f_0(\theta, x_{\omega_1}(\theta; t'_0, x'_0)) - f_0(\theta, \bar{x}(\theta; t'_0, x'_0))
      \label{eqn:proof:functional-expansion:J0}
      \\
      J_{ij}(\theta)               \coloneqq {}
      \begin{split}
         & \commutator{f_i}{f_j}(\theta, x_{\omega_1}(\theta; t'_0, x'_0)) \,  \gamma_{ij}(\omega_1) \\
         & 
        - \lim_{\omega \to \infty} \commutator{f_i}{f_j}(\theta, \bar{x}(\theta; t'_0, x'_0)) \, \gamma_{ij}(\omega)
      \end{split}
      \label{eqn:proof:functional-expansion:Jij}
    \end{align}
  \end{subequations}
  the expression
  \begingroup
  \allowdisplaybreaks
  \begin{align}
    \mathrlap{\norm{ x_{\omega_1} - \bar{x}}(t_1; t'_0, x'_0)}
    \phantom{\leq{}}
    \notag
    \\
    % \labelrel{\leq}{rel:tmp:e:1}
    %   {}
    % \begin{split}
    %    &
    %   \mathrel{\phantom{+}}
    %   \int_{t'_0}^{t_1}
    %   \norm{ J_0(\theta) } \odif{\theta}
    %   % \\
    %   % &
    %   +
    %   \int_{t'_0}^{t_1}
    %   \sum_{\mathclap{\begin{limitarray}
    %                             1 &\leq i &< l \\
    %                             i&<j&\leq l
    %                           \end{limitarray}}}
    %   \norm{J_{ij}(\theta) }
    %   \odif{\theta}                                     \\[-10pt]
    %    & + \sum_{q=0}^{r-1} \!\norm{R(t'_q, t'_{q+1})}
    %   \!+ \! \norm{R(t'_r, t_1)}
    %   \!+ \! \norm{R_{T_1}(t'_0, t_1) }
    %   \label{eqn:proof:new-approximation-lemma:23}
    % \end{split}
    % \\
    % \labelrel{\leq}{rel:tmp:e:2}
    %   {}
    % \begin{split}
    %    &
    %   \mathrel{\phantom{+}}
    %   L  \int_{t_0'}^{t_1}  \norm{ x_{\omega_1}(\theta; t'_0, x'_0) - \bar{x}(\theta; t'_0, x'_0) }  \odif{\theta}
    %   \\[-6pt]
    %    &
    %   +
    %   l(l-1) \pi  L \int_{t_s}^{t_e}  \norm{ x_{\omega_1}(\theta; t'_0, x'_0) - \bar{x}(\theta; t'_0, x'_0)} \odif{\theta} \\
    %    & +  \pi^2 {(l+1)}^3 L^2 D  \omega_1^{p'''-2} \norm{x_0'} (t_1 - t_0')                                              \\
    %    &
    %   +\pi^2 {(l+1)}^2 L^2 D \omega_1^{p'-1} \norm{ x_0' }
    %   (
    %   8 (t_1 -t_0')
    %   +12
    %   +6\pi
    %   )                                                                                                                    \\
    %    & + 2 \pi^3 {(l+1)}^3 L^2 D  \omega_1^{p'''-2} \norm{x_0'}
    % \end{split}
    % \\
    % \labelrel{\leq}{rel:tmp:e:3}
    \leq
      {}
    \begin{split}
       & 
      \mathrel{\phantom{+}}
      2 \pi l^2 L \int_{t_0'}^{t_1} \norm{ x_{\omega_1}(\theta; t'_0, x'_0) - \bar{x}(\theta; t'_0, x'_0) } \odif{\theta}
      \\
       & 
      +\pi^2 {(l+1)}^3 \! L^2 \!D \omega_1^{- p^\star} \!\! \norm{ x_0' }
      (
      9 (t_1 -t_0')
      \!+\!12
      \!+8\pi
      )
    \end{split}
    \label{eqn:proof:trajectory-approximation:error-bound}
  \end{align}
  \endgroup
  describing the norm of the error between solutions.
  %  where we
  % \begin{steps}[]
  %   \item[\eqref{rel:tmp:e:1}] use the triangle inequality to bound expressions separately,
  %   \item[\eqref{rel:tmp:e:2}] use the bounds in~\cite[Lemma~11-14]{webergharesifardebenbauer2023} respectively, and finally
  %   \item[\eqref{rel:tmp:e:3}] sum the terms up and use the definition of \( p^\star\)  in~\eqref{eqn:def:p-star}.
  % \end{steps}
  %
  Since~\eqref{eqn:proof:trajectory-approximation:error-bound} holds for every \( t_1 \in \interval[]{t'_0}{t_2}\), we may apply Grönwall's lemma to obtain
  \begin{align}
    \mathrlap{\norm{x_{\omega_1}(t_1; t'_0, x'_0) - \bar{x}(t_1; t'_0, x'_0)}}
    \phantom{aaaaaa}{} \notag
    \\
     &                                                                       %\labelrel{\leq}{rel:tmp:gl:1}
    \leq
    \pi^2 {(l+1)}^3 L^2 D \omega_1^{- p^\star} \norm{ x_0' } \, \cdot \notag \\
     & \phantom{\leq{} +}
    (
    9 (t_1 -t_0')
    +12
    +8\pi
    )
    e^{2 \pi l^2 L (t_1 - t'_0) }
    % \\
    %  & \labelrel{\leq}{rel:tmp:gl:2}
    % {(l+1)}^3 C^2 M^2 \omega_1^{-p^\star} (+ t_f +4C +3 ) e^{M(1+\frac 1 2 l(l-1)C) (t_1 - t'_0) }
  \end{align}
  for all \( t_1 \in \interval[]{t'_0}{t_2}\).
  Considering \( t_1 = t_2\) in particular, and remembering that \( t_2 - t'_0 \in \interval[open left]{0}{t_f}\) and \( \omega_1 \in \interval[open]{\omega^\star}{\infty}\), with \( \omega^\star \) defined previously, we have that
  \begin{align}
    \norm{x_{\omega_1}(t_2; t'_0, x'_0) - \bar{x}(t_2; t'_0, x'_0)} & < D \, \norm{x'_0},
  \end{align}
  which contradicts the definition of \( t_2\) in~\eqref{eqn:tmp:pfe:ca:2}. Hence, (\nameref{ass:contradiction-assumption}) is a false statement, concluding the result.
\end{proof}

\begin{proof}[of \Cref{lemma:global-exponential-stability-result}]\label{proof:global-exponential-stability-result}
  In this proof, we take the approximation property on finite intervals from \Cref{lemma:approximation-lemma}  and extend it to the infinite interval.
  
  %   Let \(t_f \in \interval[open]{0}{\infty} \) be arbitrary but fixed.
  
  With \({ \alpha \in \interval[open right]{1}{\infty}} \) and~\( \beta \in \interval[open]{0}{\infty} \) from the assumptions of this theorem,  let \( t_f \in \interval[open]{0}{\infty} \) and \(D \in \interval[open]{0}{\infty} \) be fixed and satisfying
  \begin{align}
    \bar \alpha e^{-\bar\beta t_f} +D \in \interval[open]{0}{1}.
    \label{eqn:fb1:choice-of-tf-and-d}
  \end{align}
  We observe that any time instant \( t \in \interval[open right]{t_0}{\infty} \) may be expressed as \( t = \tau + n t_f + t_0 \) with
  % \vspace{-1em}
  \vspace*{-0.5\multicolsep}
  \begin{multicols}{2}
    \noindent
    \begin{equation}
      n \coloneqq \floor*{\tfrac{t-t_0}{t_f}}
    \end{equation}
    \begin{equation}
      \tau  \coloneqq t - t_0 - n t_f
      \vphantom{\floor*{\tfrac{t-t_0}{t_f}}}
      \label{eqn:proof:lemma:ges:tau}
    \end{equation}
  \end{multicols}
  \vspace*{-0.75\multicolsep}
  \noindent
  and hence \( \tau \in \interval[open right]{0}{t_f} \).
  Then, for every \( t \in \interval[open right]{t_0}{\infty} \), there exists a unique \( t_n \coloneqq t_0 + n t_f \).
  Since \(   n  \leq \frac{t-t_0}{t_f} \leq (n+1) \) by construction,  for every \( \delta' \in \interval[open]{0}{\infty} \), we have
  \begin{align}
    e^{-\delta' (n+1)} & \leq e^{-\delta' \tfrac{t-t_0}{t_f}} \leq e^{-\delta' n}.
    \label{eqn:fb1:star}
  \end{align}
  In view of the assumptions of this theorem,~\Cref{lemma:approximation-lemma} holds in particular for initial time \( t_n \in \interval[open right]{t_0}{\infty} \) and initial condition~\( {x_n = x_{\omega}(t_n; t_0, x_0)}\) with \(\bar\Lambda = \bar\alpha\), and the chosen pair of time horizon~\(t_f\) and approximation scale~\(D\) from~\ref{eqn:fb1:choice-of-tf-and-d}, yielding an \(\omega^\star \in \interval[open]{0}{\infty}\), such that the approximation property~\eqref{eqn:lemma:approximation-lemma:approximation} holds for all \(\omega \in \interval[open]{\omega^\star}{\infty}\) and all \( t \in \interval{t_n}{t_{n+1}}\).
  
  As an intermediate step, one can inductively show that
  \begin{align}
    \norm{x_n} & \leq \norm{x_0} \, {(\bar \alpha e^{-\bar\beta t_f} + D )}^{n}. %\tag{induction hypothesis}
    \label{eqn:proof:lemma:ges:ih}
  \end{align}
  %  we prove by induction that under the conditions of this theorem,
  % \begin{description}[
  %     labelindent=0pt,
  %     font=\normalfont\footnotesize,
  %     leftmargin=0pt,
  %     topsep=0pt,
  %     partopsep = 0pt,
  %   ]
  %   \item[(Induction hypothesis)] \begin{align}
  %           \norm{x_n} & \leq \norm{x_0} \, {(\bar \alpha e^{-\bar\beta t_f} + D )}^{n}. %\tag{induction hypothesis}
  %           \label{eqn:proof:lemma:ges:ih}
  %         \end{align}
  %   \item[(Base case)]Let \( n = 0 \), then trivially \( \norm{x_0} \leq  \norm{x_0} \cdot 1 \) holds.
  %   \item[(Induction step)] Starting with \( x_{n+1} \), we see that
  %         \begin{align*}
  %           \norm{x_{n+1}}
  %            & \labelrel{\leq}{rel:tmp:ges:I:1} \bar \alpha \, \norm{x_n} \, e^{-\bar\beta t_f} + D \, \norm{x_n} = \norm{x_n} \, {(\bar \alpha e^{-\bar\beta t_f }+ D)} \\
  %            & \labelrel{\leq}{rel:tmp:ges:I:2} \norm{x_0} \, {{(\bar \alpha e^{-\bar\beta t_f} + D)}^{n+1}},
  %         \end{align*}
  %         where we
  %         \begin{steps}
  %           \item[\eqref{rel:tmp:ges:I:1}] use the exponential stability of~\eqref{eqn:lbs} and the approximation property on finite intervals~\eqref{eqn:lemma:approximation-lemma:approximation} from \Cref{lemma:approximation-lemma},
  %           \item[\eqref{rel:tmp:ges:I:2}] then insert the induction hypothesis~\eqref{eqn:proof:lemma:ges:ih},
  %         \end{steps}
  %         which yields the claimed hypothesis and concludes the induction step.
  % \end{description}
  
  
  Finally, we are ready to prove the statement of this theorem. A sequence of calculations shows
  \begin{subequations}
    \begin{align*}
      \norm{x(t; t_0, x_0)}
       & \labelrel{\leq}{rel:tmp:lemma:ges:1} \norm{x_n} \, {( \bar \alpha  e^{-\bar\beta (t-t_n)} +D)}                                                               \\
       & \labelrel{=}{rel:tmp:lemma:ges:2} \norm{x_n} {( \bar \alpha e^{-\bar\beta \tau} +D)}                                                                         \\
       & \labelrel{\leq}{rel:tmp:lemma:ges:3} \norm{x_0} \,  {(\bar \alpha e^{-\bar\beta t_f} +D)}^{n} {(\bar \alpha e^{-\bar\beta \tau} + D)}                        \\
       & =  \norm{x_0} \,   {(\bar \alpha e^{-\bar\beta t_f} + D)}^{n+1}  \smash[b]{\tfrac{(\bar \alpha e^{-\bar\beta \tau} + D)}{\bar \alpha e^{-\bar\beta t_f}+ D}} \\
       & \labelrel{\leq}{rel:tmp:lemma:ges:5} \alpha \, \norm{x_0} \,  e^{-\beta (t-t_0)}
    \end{align*}
  \end{subequations}
  the claimed global uniform exponential stability with \( \alpha \) and \( \beta \) defined as
  \begin{align}
    \alpha & \coloneqq \frac{ \bar \alpha +D}{\bar \alpha e^{-\bar\beta t_f}+D} \qquad\text{and}\label{eqn:lemma:ges:alpha} \\
    \beta  & \coloneqq -\frac{1}{t_f} \ln(\bar \alpha e^{-\bar\beta t_f}+D), \label{eqn:lemma:ges:beta}
  \end{align}
  respectively, where we use
  \begin{steps}
    \item[\eqref{rel:tmp:lemma:ges:1}] the exponential stability of~\eqref{eqn:lbs} and the approximation property on finite intervals from~\Cref{lemma:approximation-lemma},
    \item[\eqref{rel:tmp:lemma:ges:2}] definitions of \( t \), \( t_n\) and \( \tau \) from~\eqref{eqn:proof:lemma:ges:tau},
    \item[\eqref{rel:tmp:lemma:ges:3}]  inequality~\eqref{eqn:proof:lemma:ges:ih} from the previous inductive scheme and
    \item[\eqref{rel:tmp:lemma:ges:5}] the fact that \(e^{-\bar \beta \tau} \leq 1\),~\eqref{eqn:fb1:star} and definitions~(\ref{eqn:lemma:ges:alpha}-\ref{eqn:lemma:ges:beta}).\qedhere
  \end{steps}
  % Under the conditions of this lemma, for all \( t_0 \in \mathbb{R} \) and for all \( x_0 \in \mathbb{R} \),
  % \begin{align}
  % 	\norm{x(t; t_0, x_0)} & \leq \gamma \norm{x_0}e^{-\delta (t-t_0)}
  % 	\qquad\text{for all \( t \in \interval[open right]{t_0}{\infty}, \)}
  % \end{align}
  % i.e.\ the origin is globally practically exponentially stable for~\eqref{eqn:fb1:es}.
\end{proof}

\begin{proof}[of \Cref{lemma:frequency-adaptation}]\label{proof:frequency-adaptation}
  The Lie-bracket system of form~\eqref{eqn:lbs} associated with~\eqref{eqn:augmented-system:state} remains the same for all \( w_k \in \interval[open]{0}{\infty}\).
  Since the origin is globally exponentially stable with respect to~\eqref{eqn:lbs} associated with~\eqref{eqn:augmented-system:state} due to the assumptions of this lemma, in view of \Cref{lemma:global-exponential-stability-result}, there exists a \(\omega^\star \in \interval[open]{0}{\infty}\), such that for all \( w_k \in \interval[open]{\omega^\star}{\infty}\), the origin is globally uniformly  exponentially stable with respect to~\eqref{eqn:augmented-system:state}.
  
  Consider a solution \(w(t; t_0, w_0)\) to~\eqref{eqn:augmented-system:frequency}, which is monotonically increasing by construction. Hence, either \(w(t; t_0, w_0)\) grows unbounded, or \(w(t; t_0, w_0)\) is bounded.
  
  Assume with contradiction intent, that \(w(t; t_0, w_0)\) grows unbounded.
  As solutions to~\eqref{eqn:augmented-system:frequency} exist globally due to the global Lipschitz properties from \Cref{ass:fi}, there exists a \( k^\star \in \mathbb{N}\), such that \( w(t; t_k, w_k) \geq \omega^\star\) for all \( k \geq k^\star\).
  Hence, the solutions \( x_{w_{k}}(t; t_{k}, x_{k})\) exponentially converge to zero for \( k \geq k^\star\), and \( x_{k^\star}\) is finite.
  Consequently, it can be shown by simple integration of~\eqref{eqn:augmented-system:frequency}, that \(w(t; t_{k^\star}, x_{k^\star})\) has a finite limit, which contradicts our initial assumption.
  
  Hence, finite escape time of \(w(t; t_0, w_0)\) is excluded and the statement of this lemma follows.
\end{proof}

% do not print the proofs of the auxiliary lemmata for the conference versions
% \subsection{Proofs of Auxiliary Results}
% 	% \pagebreak
% 	\printProofs[auxiliary-result]

% \subsection{Proofs of Example Results}
% 	% \pagebreak
% 	\printProofs[lipschitz-proofs]

==> src/sections/simulation-example/00--simulation-example.tex <==
We demonstrate the importance of \Cref{lemma:global-exponential-stability-result} using an example from adaptive control.

\begin{description}[
    labelindent=0pt,
    % font=\normalfont\footnotesize,
    leftmargin=0pt,
    topsep=0.5em,
    % partopsep = 0pt,
    itemsep=0.5em,
  ]
  \item[System Dynamics]
        Consider the scalar linear time-invariant system
        \begin{subequations}\label{eqn:example-system}
          \begin{align}
            \dot{x}(t) = {} & a x(t) + b u(t, x(t))
            \label{eqn:example-system:dynamics}
            \\
            u(t, x) = {}
            \begin{split}
               & {}\mathrel{\phantom{+}} \sqrt{\omega}\, k^{\tfrac 1 2} |x| \sin( \log(\tfrac 1 2 x^2)) \sin(\omega t) \\
               & {}+ \sqrt{\omega} \, k^{\tfrac 1 2} |x| \cos( \log(\tfrac 1 2 x^2)) \cos(\omega t)
            \end{split}
          \end{align}
        \end{subequations}
        with \( a \in \mathbb{R}\), \(b \in \mathbb{R}\!\setminus\!\set{0}\) unknown, yet with \(k\) sufficiently large, i.e.\ \( k \in \interval[open]{\tfrac{a}{b^2}}{\infty}\).
        By convention, let \(|x| \sin( \log(\frac 1 2 x^2)) |_{x=0} = |x| \cos( \log(\frac 1 2 x^2)) |_{x=0} = 0\).
        % \end{example}
  \item[Numerical Setup]
        We simulate system~\eqref{eqn:example-system} with \( {t \in \interval[]{\SI{0}{\second}}{\SI{10}{\second}}}\), \({ \omega = \SI{200}{\radian\per\second}}\), \( {a= 2}\), \({ b = -3}\) and \({ k = \tfrac 1 2}\) using an \textit{ode1}-solver with stepwidth~\({h=\SI{1e-4}{\second}}\).
  \item[Expected Results]
        System~\eqref{eqn:example-system} is in the form~\eqref{eqn:es-system} with vector fields
        \begin{subequations}
          \label{eqn:example-system:vectorfields}
          \begin{align}
            f_0(t, x) & = a x,
            \label{eqn:example-system:0}                                                                   \\
            f_1(t, x) & = bk^{\tfrac 1 2} |x| \sin( \log (\tfrac 1 2 x^2) ), 	\label{eqn:example-system:1} \\
            f_2(t, x) & = bk^{\tfrac 1 2} |x| \cos( \log (\tfrac 1 2 x^2) ),
            \label{eqn:example-system:2}
          \end{align}
          powers \( p_0 = 0\), \( p_1 = p_2 = \tfrac 1 2\) and dither signals
          % \vspace{-0.75em}
          \begin{multicols}{2}
            \noindent
            \begin{equation}
              u_1(s) = \sin(s),
            \end{equation}
            \begin{equation}
              u_2(s) = \cos(s)
            \end{equation}
          \end{multicols}
          % \vspace{-0.75em}
          \noindent
          and satisfies \Cref{ass:ui,ass:fi,ass:pi} with \( L  \leq 2838\), as shown in \cite[Lemma~15-17]{webergharesifardebenbauer2023}.
        \end{subequations}
        The associated Lie-bracket system is
        \begin{align}
          \bar{x}(t) & = (a-b^2 k)\bar{x}(t),
          \label{eqn:example:lbs}
        \end{align}
        which can easily be shown to be uniformly exponentially stable for our choice of values \( k \in \interval[open]{\tfrac{a}{b^2}}{\infty}\) .
        Moreover, we may select \(\bar{\alpha} = 1\) and \(\bar{\beta} = b^2 k - a\).
        % \vspace{-0.5ex}
        % \begin{subequations}
        %   % \abovedisplayskip=0pt
        %   % \abovedisplayshortskip=0pt
        %   \begin{multicols}{2}
        %     \noindent
        %     \begin{equation}
        %       \bar{\alpha} = 1
        %     \end{equation}
        %     \begin{equation}
        %       \bar{\beta} = b^2 k - a.
        %     \end{equation}
        %   \end{multicols}
        % \end{subequations}
        % \vspace{-0.5ex}
        Then, for any \( k \in \interval[open]{\tfrac{a}{b^2}}{\infty}\), any \( t_f \in \interval[open]{0}{\infty}\), we may choose \(D  = \tfrac 1 2 (e^{-\bar \beta t_f} -1)\)
        % \linebreak
        % \vspace*{-2ex}
        % \begin{align}
        %   D & = \tfrac 1 2 (e^{-\bar \beta t_f} -1)
        % \end{align}
        to satisfy~\eqref{eqn:fb1:choice-of-tf-and-d}. Accordingly, we can select a sufficiently large \( \omega^\star\) using~\eqref{eqn:def:omega-star}.
        
        
        \Cref{lemma:global-exponential-stability-result} asserts, that for all \( \omega \in \interval[open]{\omega^\star}{\infty}\), the system~\eqref{eqn:example-system} is uniformly globally exponentially stable, and we expect our simulation results to reflect this;
        We wish to emphasize that this conclusion cannot be drawn from any of the existing results in the literature.
        % Then there exists an \( \omega^\star \in \interval[open]{0}{\infty}\), such that for all \( \omega \in \interval[open]{\omega^\star}{\infty}\), the origin is uniformly globally exponentially stable with respect to \eqref{eqn:example-system}.
        
        
        
        % We demonstrate the solution using \eqref{eqn:example-system} with \( a = 2\), \( b = 3\) for different values of \(k\).
  \item[Observations]
        The resulting trajectories are shown in \Cref{fig:simulation-result}.
        Observe, that the hull of the solution to the example system~\eqref{eqn:example-system}~(\ref{plot:exponential-convergence:ai}) is described by an exponentially decaying curve~(\ref{plot:exponential-convergence:upperbound-emprical}), which contains the curve of the associated Lie-bracket system~\eqref{eqn:example:lbs}~(\ref{plot:exponential-convergence:lbs}).
        Notably, the convergence rate of~\(x_{\omega}(t; t_0, x_0)\) seems to be proportional to \( - \bar\beta\)~(\ref{plot:exponential-convergence:upperbound-emprical}) instead of the calculated rate~\(-\beta\)~(\ref{plot:exponential-convergence:upperbound-analytical}), which indicates a faster convergence than postulated.
        The rate of convergence may be tuned further using different values of \( k\).
\end{description}
\begin{figure}
  \centering
  % \includegraphics[width=\linewidth]{src/sections/simulation-example/simulation-figure.tikz}
  \input{src/sections/simulation-example/simulation-figure.tikz}
  \caption{Simulation results show the solution~\(x_{\omega}(t; t_0, x_0)\)~(\ref{plot:exponential-convergence:ai}) from~\eqref{eqn:example-system}, the solution~\(\bar{x}(t; t_0, x_0)\)~(\ref{plot:exponential-convergence:lbs}) of the associated Lie-bracket system~\eqref{eqn:example:lbs} for a common initial condition \(x_0\), the conservative analytical upper bound~\(\alpha e^{-\beta t}\)~(\ref{plot:exponential-convergence:upperbound-analytical}) as well as the empirical  bounds~\( \alpha e^{-\bar{\beta} t}\)~(\ref{plot:exponential-convergence:upperbound-emprical}) for parameters from \Cref{sec:simulation-example}.}
  \label{fig:simulation-result}
\end{figure}


